Generating Signed Language Instructions in Large-Scale Dialogue Systems

We introduce a goal-oriented conversational AI system enhanced with American Sign Language (ASL) instructions, presenting the first implementation of such a system on a worldwide multimodal conversational AI platform. Accessible through a touch-based interface, our system receives input from users and seamlessly generates ASL instructions by leveraging retrieval methods and cognitively based gloss translations. Central to our design is a sign translation module powered by Large Language Models, alongside a token-based video retrieval system for delivering instructional content from recipes and wikiHow guides. Our development process is deeply rooted in a commitment to community engagement, incorporating insights from the Deaf and Hard-of-Hearing community, as well as experts in cognitive and ASL learning sciences. The effectiveness of our signing instructions is validated by user feedback, achieving ratings on par with those of the system in its non-signing variant. Additionally, our system demonstrates exceptional performance in retrieval accuracy and text-generation quality, measured by metrics such as BERTScore. We have made our codebase and datasets publicly accessible at https://github.com/Merterm/signed-dialogue, and a demo of our signed instruction video retrieval system is available at https://huggingface.co/spaces/merterm/signed-instructions.

==> todo.tex <==
-we need to make it clear and frame it from the perspective that if you average all the participants then you lose the meaning of the eye gaze. This is important to show. But do not frame it as we are only showing a single person's images, as that is anecdotal. We are using this as a tool to plot the eye gazes of people in terms of areas in a picture, and show their differences. This is a big contribution in the eye gaze community. We provide the python package for it. We also show that discourse goals change the eye gaze patterns. We show this with three experiments in discourse.
